ChineseSafe: A Chinese Benchmark for Evaluating Safety in Large Language Models

With the rapid development of Large language models (LLMs), understanding the capabilities of LLMs in identifying unsafe content has become increasingly important. While previous works have introduced several benchmarks to evaluate the safety risk of LLMs, the community still has a limited understanding of current LLMs' capability to recognize illegal and unsafe content in Chinese contexts. In this work, we present a Chinese safety benchmark (ChineseSafe) to facilitate research on the content safety of large language models. To align with the regulations for Chinese Internet content moderation, our ChineseSafe contains 205,034 examples across 4 classes and 10 sub-classes of safety issues. For Chinese contexts, we add several special types of illegal content: political sensitivity, pornography, and variant/homophonic words. Moreover, we employ two methods to evaluate the legal risks of popular LLMs, including open-sourced models and APIs. The results reveal that many LLMs exhibit vulnerability to certain types of safety issues, leading to legal risks in China. Our work provides a guideline for developers and researchers to facilitate the safety of LLMs. Our results are also available at https://huggingface.co/spaces/SUSTech/ChineseSafe-Benchmark. Additionally, we release a test set comprising 200,000 examples, which is publicly accessible at https://huggingface.co/datasets/SUSTech/ChineseSafe.

==> table/new_prompt_gen_sub/main_gen.tex <==
\begin{table}[t]
	\centering
	\caption{The main results (\%) on the test split under diverse LLMs using generation for assessment.}
	% \scriptsize
        \footnotesize
        \renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{4mm}\begin{tabular}{lccccc}
		\toprule
		\multirow{2}*{Model} & \multirow{2}{*}{Accuracy}  & \multicolumn{2}{c}{Unsafe} & \multicolumn{2}{c}{Safe} \\
		& & Precision & Recall & Precision & Recall  \\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}    \\  
		\midrule
            DeepSeek-LLM-67B-Chat &77.07/0.91&72.48/1.28&86.92/0.86&86.03/0.90&67.09/1.20
\\
            Llama3-ChatQA-1.5-70B &68.67/1.16&66.03/1.15&75.78/1.31&73.02/1.50&61.42/1.78
\\
            Qwen1.5-72B-Chat &70.59/1.13&72.23/1.87&60.64/2.04&69.46/1.40&80.45/0.95
\\
            Opt-66B &53.94/1.29&52.71/1.35&79.46/1.34&58.15/1.97&28.26/1.39
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}    \\  
		\midrule
            Yi-1.5-34B-Chat &72.85/0.91&73.26/1.53&68.32/1.39&74.43/1.28&77.17/1.21
\\
            Opt-30B &50.80/1.23&50.67/1.16&73.38/1.50&51.26/2.34&28.06/1.95
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}    \\  
		\midrule
		  InternLM2-Chat-20B &75.57/1.07&76.89/1.49&71.34/2.06&76.18/1.51&79.62/1.09
\\
            Qwen1.5-14B &72.76/1.01&67.74/1.40&84.73/1.01&83.89/1.02&60.57/1.49
\\
            Baichuan2-13B-Chat &67.39/1.28&66.18/1.43&67.67/1.73&69.06/1.55&66.94/2.11
\\
            Ziya2-13B-Chat &57.96/1.08&56.29/1.20&64.40/1.43&61.35/1.77&51.33/1.25
\\
            Opt-13B &50.72/1.07&50.61/1.20&71.22/1.76&51.14/1.72&30.07/1.21
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}    \\  
		\midrule
            Gemma-1.1-7B &74.54/0.98&69.36/1.33&86.59/1.13&84.88/1.19&62.25/1.31
\\
            DeepSeek-LLM-7B-Chat &75.73/0.84&69.85/1.19&90.28/0.81&87.59/1.07&61.00/1.20
\\
            GLM-4-9B-Chat &74.38/0.94&83.24/1.91&54.32/1.14&71.00/1.17&94.41/0.89
\\
            Mistral-7B &75.96/0.94&70.14/1.03&90.61/0.76&87.24/1.17&61.21/1.44
\\
            Qwen1.5-7B-Chat &66.16/0.79&60.42/1.19&88.30/0.95&85.51/1.26&43.85/1.01
\\
            Yi-1.5-9B-Chat &74.24/1.05&71.18/1.19&81.36/1.28&79.54/1.42&67.13/1.52
\\
            Llama3-ChatQA-1.5-8B &60.79/1.03&56.84/1.03&91.32/0.82&78.25/2.14&30.09/1.20
\\
            Baichuan2-7B &59.09/1.03&63.65/1.75&37.33/1.68&57.21/1.07&81.16/0.96
\\
            InternLM2-chat-7B &66.70/1.04&68.28/1.59&60.60/1.66&65.94/1.24&72.72/1.05
\\
            GPT-J-6B &57.42/1.26&55.35/1.27&77.95/1.43&62.88/1.98&36.83/1.93
\\
            Opt-6.7B &50.38/1.03&50.40/1.14&68.61/1.25&50.39/2.13&32.02/1.96
\\
		\bottomrule
	\end{tabular}
	\vspace{-1.0em}
 
	\label{main_gen}
\end{table}

==> table/new_prompt_gen_sub/sub_gen_ethics.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: ethics and morality}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclccllll}
 & \multicolumn{9}{c}{Ethics and Morality}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{DIS}& \multicolumn{3}{c}{SWE}&  \multicolumn{3}{c}{ETH}\\
        ~ & acc& P&R& acc& P& R& acc& P&R\\ 
        \midrule
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 75.82& 68.29&94.24
& 86.2& 78.79& 98.28
& 71.73& 71.7&73.88
\\
		Llama3-ChatQA-1.5-70B & 74.06& 68.56&86.87
& 78.1& 72.24& 90.01
& 61.19& 61.9&62.77
\\
		Qwen1.5-72B-Chat & 73.96& 73.37&73.39
& 82.59& 85.06& 78.11
& 55.65& 61.88&34.34
\\
		Opt-66B & 49.85& 49.14&71.19
& 55.9& 53.15& 84.41
& 52.44& 52.43&74.91
\\
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 78.48& 79.66&75.25
& 85.52& 82.91& 88.71
& 53.4& 59.1&28.52
\\
 Opt-30B & 45.24& 45.77& 65.39
& 53.18& 51.46& 78.08
& 49.89& 50.71&71.09
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 77.74& 79.74& 73.06
& 88.26& 83.44& 94.85
& 56.47& 63.92&33.94
\\
 Qwen1.5-14B 
& 75.2& 68.16& 92.42
& 83.51& 75.6& 97.96
& 59.4& 60.85&57.71
\\
 Baichuan2-13B-Chat 
& 72.15& 70.08& 75.27
& 78.18& 73.59& 86.58
& 63.29& 64.5&62.84
\\
 Ziya2-13B-Chat 
& 59.8& 57.05& 71.91
& 63.74& 58.45& 89.95
& 42.32& 41.91&33.31
\\
		Opt-13B & 45.69& 45.91&62.16
& 53.04& 51.42& 75.72
& 48.12& 49.43&66.19
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 77.06& 69.84& 93.38
& 76.82& 68& 99.52
& 67.28& 66.08&74.09
\\
 DeepSeek-LLM-7B-Chat 
& 75.2& 69.99& 86.33
& 80.34& 71.49& 99.6
& 65.71& 65.37&70.07
\\
 GLM-4-9B-Chat 
& 81.81& 91.82& 68.97
& 93.18& 95.4& 90.39
& 52.36& 68.55&12.64
\\
 Mistral-7B 
& 78.4& 70.74& 95.21
& 80.33& 71.45& 99.66
& 69.13& 67.06&77.96
\\
 Qwen1.5-7B-Chat 
& 72.93& 66.26& 91
& 70.78& 62.79& 99.1
& 42.57& 42.39&34.71
\\
 Yi-1.5-9B-Chat 
& 81.52& 78.15& 86.35
& 87.27& 81.62& 95.49
& 55.05& 56.37&53.8
\\
 Llama3-ChatQA-1.5-8B 
& 60.64& 55.59& 97.11
& 65.66& 59& 98.25
& 57.07& 55.37&82.86
\\
 Baichuan2-7B 
& 56.65& 63.53& 26.75
& 67.11& 68.05& 61.85
& 45.22& 38.39&11.67
\\
 InternLM2-chat-7B 
& 69.28& 75.58& 55.03
& 82.74& 81.08& 84.44
& 52.32& 54.31&42.59
\\
 GPT-J-6B 
& 55.34& 53.08& 75.48
& 60.65& 56.46& 86.38
& 50.07& 50.95&62.23
\\
 Opt-6.7B & 46.49& 46.4& 60.63
& 51.02& 50.02& 71.68
& 50.49& 51.23&66.65
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/new_prompt_gen_sub/sub_gen_health.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: Health and Privacy}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclcclllllll}
 & \multicolumn{9}{c}{Health and Privacy} & \multicolumn{3}{c}{Variants}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{Phy}& \multicolumn{3}{c}{Men}&  \multicolumn{3}{c}{Pri} & \multicolumn{3}{c}{}\\
        ~ & acc& P&R& acc& P& R& acc& P&R & acc& P&R \\ 
        \midrule
		\multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 63.86& 64.74&57.96
& 71.89& 72.14& 70.12
& 74.51& 68.72&87.82
& 80.6& 73.15&98.2
\\
		Llama3-ChatQA-1.5-70B & 55.99& 57.07&42.41
& 67.45& 63.74& 79.1
& 64.82& 61.7&74.01
& 66.96& 66.29&72.24
\\
		Qwen1.5-72B-Chat & 48.42& 40.95&11.31
& 58.57& 63.46& 37.4
& 66.89& 71.86&53.09
& 77.48& 75.26&83.47
\\
		Opt-66B & 53.82& 51.95&80.76
& 54.09& 52.24& 80.74
& 55.5& 52.77&85.28
& 52.84& 52.8&74.67
\\
		\multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 54.24& 57.92&24.81
& 63.73& 70.32& 45.95
& 72.06& 74.3&65.52
& 75.42& 70.02&90.93
\\
 Opt-30B & 48.37& 48.32& 71.9
& 51.36& 50.51& 75.37
& 51.87& 50.51&76.38
& 50.88& 51.48&70.83
\\
 \multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 64.68& 72.03& 45.94
& 68.13& 73.56& 55.01
& 73.22& 79.57&60.87
& 76.13& 76.02&77.98
\\
 Qwen1.5-14B 
& 54.3& 54.78& 39.55
& 77.59& 69.47& 97.37
& 68.22& 63.54&82.23
& 73.29& 66.29&97.4
\\
 Baichuan2-13B-Chat 
& 50.93& 50.07& 27.4
& 56.75& 58.19& 44.36
& 68.69& 64.89&78.43
& 64.72& 65.06&67.19
\\
 Ziya2-13B-Chat 
& 54.65& 54.02& 51.73
& 53.99& 54.06& 45.4
& 48.31& 47.15&48
& 62.68& 61.73&71.51
\\
		Opt-13B & 50.5& 49.75&73.28
& 52.86& 51.5& 75.73
& 51.35& 50.13&73.94
& 50.87& 51.5&70.13
\\
 \multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 56.14& 56.25& 47.55
& 78.16& 70.35& 96.39
& 69.11& 65.02&79.64
& 80.38& 74.74&93.24
\\
 DeepSeek-LLM-7B-Chat 
& 73.2& 67.46& 87.9
& 71.87& 68.24& 80.35
& 73.03& 66.5&90.23
& 79.11& 72.37&95.78
\\
 GLM-4-9B-Chat 
& 51.77& 60.14& 5.83
& 51.44& 58.9& 5.6
& 69.65& 86.39&45.01
& 76& 91.47&58.61
\\
 Mistral-7B 
& 70.55& 66.69& 80.1
& 76.35& 70.94& 88.2
& 73.59& 67.01&90.55
& 75.49& 70.23&90.57
\\
 Qwen1.5-7B-Chat 
& 64.63& 59.12& 90.96
& 61.2& 58.06& 77.25
& 66.47& 60.21&92.51
& 70.91& 63.87&99.5
\\
 Yi-1.5-9B-Chat 
& 66.94& 68.68& 60.21
& 76.75& 70.21& 91.9
& 70.47& 65.05&85.58
& 68.84& 68.59&72.37
\\
 Llama3-ChatQA-1.5-8B 
& 54.82& 52.53& 83.58
& 57.5& 54.14& 91.29
& 57.48& 54&87.7
& 60.22& 56.79&93.48
\\
 Baichuan2-7B 
& 51.4& 51.39& 20.64
& 63.3& 75.58& 37.71
& 58.82& 69.06&28.57
& 60.31& 66.31&45.73
\\
 InternLM2-chat-7B 
& 53.98& 56.48& 27.63
& 61.13& 62.21& 54.04
& 61.22& 62.6&51.28
& 69.42& 68.29&75.31
\\
 GPT-J-6B 
& 58.36& 55.22& 80.9
& 58.68& 55.64& 80.43
& 57.46& 54.45&78.73
& 58.44& 56.81&78.72
\\
 Opt-6.7B & 49.66& 49.14& 68.97
& 48.88& 48.71& 67.83
& 50.57& 49.6&68.89
& 50.24& 51.09&67.23
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/new_prompt_gen_sub/sub_gen_illegal.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: illegal activities}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclccllll}
 & \multicolumn{9}{c}{Illegal activities}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{PI}& \multicolumn{3}{c}{POR}&  \multicolumn{3}{c}{CRI}\\
        ~ & acc& P&R& acc& P& R& acc& P&R\\ 
        \midrule
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 84.74& 79.79&96.51
& 85.31& 79.77& 95.58
& 75.99& 67.67&96.66
\\
		Llama3-ChatQA-1.5-70B & 71.23& 69.2&85.02
& 71.9& 70.58& 77.62
& 74.98& 69.02&87.79
\\
		Qwen1.5-72B-Chat & 79.47& 84.41&76.35
& 80.44& 85.8& 74.2
& 82.46& 80.22&84.76
\\
		Opt-66B & 56.72& 57.39&79.62
& 54.55& 53.86& 79.88
& 53.65& 51.36&83.17
\\
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 80.02& 78.34&87.51
& 82.58& 83.06& 82.98
& 83.12& 76.98&93.03
\\
 Opt-30B & 54.15& 55.91& 74.8
& 51.58& 52.01& 74.7
& 51.49& 50.02&75.26
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 84.45& 81.27& 92.86
& 85.98& 83.63& 90.44
& 80.66& 75.75&88.42
\\
 Qwen1.5-14B 
& 77.5& 71.94& 96.24
& 84.41& 80.21& 92.43
& 74.2& 66.57&94.02
\\
 Baichuan2-13B-Chat 
& 73.54& 73.06& 81.43
& 69.8& 69.97& 72.13
& 75.86& 72.41&81.05
\\
 Ziya2-13B-Chat 
& 64.4& 63.23& 82.78
& 69.38& 68.25& 75.42
& 60.36& 57.05&73.95
\\
		Opt-13B & 53.24& 55.45&71.82
& 52.51& 52.71& 72.77
& 49.05& 48.3&70.46
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 76.21& 70.85& 95.69
& 85.27& 80.09& 94.91
& 78.95& 72.36&91.53
\\
 DeepSeek-LLM-7B-Chat 
& 79.95& 73.71& 98.19
& 80.81& 73.36& 98.29
& 78.09& 70&96.01
\\
 GLM-4-9B-Chat 
& 88.92& 95.6& 83.5
& 88.78& 94.58& 82.96
& 89.9& 89.54&89.68
\\
 Mistral-7B 
& 77.74& 73.21& 93.25
& 81.39& 75.93& 93.33
& 76.62& 68.14&97.32
\\
 Qwen1.5-7B-Chat 
& 72.77& 66.92& 98.86
& 69.23& 62.54& 99.81
& 70.16& 62.02&99.32
\\
 Yi-1.5-9B-Chat 
& 77.7& 75.51& 87.39
& 78.43& 76.23& 84.22
& 79.45& 71.36&96.26
\\
 Llama3-ChatQA-1.5-8B 
& 63.53& 60.98& 91.7
& 67.45& 62.68& 90.43
& 63.54& 57.36&96.83
\\

 Baichuan2-7B 
& 47.06& 54.27& 17.36
& 70.37& 73.91& 65.1
& 70.71& 75.99&57.88
\\
 InternLM2-chat-7B 
& 68.7& 73.26& 66.95
& 74.91& 79.43& 68.98
& 73.31& 69.57&79.8
\\
 GPT-J-6B 
& 59.58& 60.04& 77.16
& 58.77& 57.23& 77.65
& 56.83& 53.59&81.77
\\
 Opt-6.7B & 53.07& 55.52& 69.55
& 52.94& 53.03& 72.66
& 50.49& 49.29&71.98
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/new_prompt_gen_total/main_gen.tex <==
\begin{table}[t]
	\centering
	\caption{The main results (\%) on the test split under diverse LLMs using generation for assessment.}
	% \scriptsize
        \footnotesize
        \renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{4mm}\begin{tabular}{lccccc}
		\toprule
		\multirow{2}*{Model} & \multirow{2}{*}{Accuracy}  & \multicolumn{2}{c}{Unsafe} & \multicolumn{2}{c}{Safe} \\
		& & Precision & Recall & Precision & Recall  \\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}    \\  
		\midrule
            DeepSeek-LLM-67B-Chat &73.14/0.32&70.06/0.24&81.40/0.82&77.49/0.64&64.78/0.35
\\
            Llama3-ChatQA-1.5-70B &62.31/0.79&61.68/0.87&66.25/0.57&63.06/0.70&58.33/1.01
\\
            Qwen1.5-72B-Chat &72.06/0.51&74.16/0.46&68.23/0.80&70.25/0.53&75.93/0.29
\\
            Opt-66B &54.64/0.57&53.32/0.31&78.98/1.12&58.53/1.46&30.00/0.37
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}    \\  
		\midrule
            Yi-1.5-34B-Chat &66.29/0.21&71.60/0.25&54.67/0.31&62.97/0.19&78.05/0.25
\\
            Opt-30B &51.53/0.05&51.28/0.12&73.33/0.39&52.19/0.13&29.47/0.42
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}    \\  
		\midrule
		  InternLM2-Chat-20B &73.04/0.27&73.50/0.51&72.58/0.17&72.59/0.11&73.51/0.58
\\
            Qwen1.5-14B &65.14/0.41&64.04/0.42&70.05/0.72&66.50/0.51&60.18/0.40
\\
            Baichuan2-13B-Chat &64.63/0.28&63.22/0.34&70.99/0.65&66.46/0.28&58.19/0.63
\\
            Ziya2-13B-Chat &57.66/0.51&56.11/0.46&72.72/0.34&60.57/0.62&42.43/0.81
\\
            Opt-13B &50.86/0.19&50.83/0.19&70.47/0.88&50.93/0.27&31.01/0.57
\\
		\midrule
		\multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}    \\  
		\midrule
            Gemma-1.1-7B &68.53/0.66&65.47/0.47&79.22/1.14&73.30/1.05&57.71/0.19
\\
            DeepSeek-LLM-7B-Chat &69.88/0.20&69.64/0.25&71.14/0.29&70.13/0.14&68.61/0.21
\\
            GLM-4-9B-Chat &74.60/0.16&89.14/0.02&56.37/0.48&67.81/0.14&93.04/0.10
\\
            Mistral-7B &71.71/0.12&68.02/0.08&82.60/0.28&77.50/0.24&60.68/0.16
\\
            Qwen1.5-7B-Chat &68.09/0.42&62.45/0.34&91.70/0.42&84.02/0.72&44.18/0.35
\\
            Yi-1.5-9B-Chat &69.76/0.42&65.38/0.35&84.79/0.37&77.98/0.50&54.55/0.68
\\
            Llama3-ChatQA-1.5-8B &62.10/0.17&57.60/0.18&93.40/0.15&81.99/0.25&30.41/0.21
\\
            Baichuan2-7B &59.00/0.23&63.15/0.48&44.43/0.12&56.73/0.14&73.75/0.44
\\
            InternLM2-chat-7B &61.77/0.19&73.44/0.62&37.59/0.22&57.72/0.07&86.23/0.34
\\
            GPT-J-6B &58.06/0.29&55.98/0.27&77.86/0.15&62.91/0.39&38.02/0.56
\\
            Opt-6.7B &50.88/0.20&50.86/0.10&69.59/0.44&50.92/0.48&31.94/0.16
\\
		\bottomrule
	\end{tabular}
	\vspace{-1.0em}
 
	\label{main_gen}
\end{table}

==> table/new_prompt_gen_total/sub_gen_ethics.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: ethics and morality}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclccllll}
 & \multicolumn{9}{c}{Ethics and Morality}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{DIS}& \multicolumn{3}{c}{SWE}&  \multicolumn{3}{c}{ETH}\\
        ~ & acc& P&R& acc& P& R& acc& P&R\\ 
        \midrule
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 77.92& 71.56&91.13
& 81.27& 73.09& 97.83
& 65.12& 65.04&64.89
\\
		Llama3-ChatQA-1.5-70B & 68.89& 65.47&77.26
& 76.09& 69.37& 91.85
& 52.36& 52.72&43.85
\\
		Qwen1.5-72B-Chat & 74.76& 74.21&74.37
& 83.66& 78.17& 92.5
& 62.71& 66.83&50.19
\\
		Opt-66B & 51.18& 50.12&73.24
& 55.82& 53.21& 82.5
& 52.16& 51.47&74.52
\\
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 65.58& 70.73&50.7
& 80.22& 79.44& 80.55
& 49.24& 47.79&18.51
\\
 Opt-30B & 48.3& 48.02& 67.11
& 53.7& 51.87& 77.96
& 50.67& 50.4&71.16
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 72.7& 72.42& 71.38
& 83.12& 77.39& 92.65
& 59.82& 63.55&45.68
\\
 Qwen1.5-14B 
& 71.56& 67.01& 82.47
& 79.66& 71& 98.98
& 43.86& 40.37&26.53
\\
 Baichuan2-13B-Chat 
& 66.81& 64.3& 72.63
& 76.71& 69.76& 92.67
& 58.49& 58.9&55.64
\\
 Ziya2-13B-Chat 
& 59.31& 56.14& 77.42
& 61.49& 57.59& 81.73
& 48.53& 48.61&55.14
\\
		Opt-13B & 47.59& 47.41&64.15
& 52.14& 50.87& 73.39
& 48.21& 48.57&64.86
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 73.37& 67.36& 88.49
& 78.82& 70.01& 99.45
& 61.04& 60.47&63.21
\\
 DeepSeek-LLM-7B-Chat 
& 65.11& 65.54& 60.66
& 81.55& 74.79& 94.11
& 51.94& 52.8&34.38
\\
 GLM-4-9B-Chat 
& 82.98& 90.78& 72.64
& 94.7& 92.93& 96.51
& 53.75& 67.12&14.36
\\
 Mistral-7B 
& 75.59& 69.61& 89
& 80.62& 71.95& 99.19
& 69.78& 67.26&76.84
\\
 Qwen1.5-7B-Chat 
& 67.94& 61.77& 90.72
& 71.48& 63.63& 97.75
& 59.9& 57.68&73.7
\\
 Yi-1.5-9B-Chat 
& 74.91& 67.37& 94.44
& 77.43& 68.62& 99.52
& 64& 62.01&71.89
\\
 Llama3-ChatQA-1.5-8B 
& 61.91& 56.67& 94.59
& 64.31& 57.97& 99.31
& 59.06& 55.7&87.61
\\
 Baichuan2-7B 
& 57.41& 59.98& 39.26
& 59.77& 62.88& 44.09
& 49.3& 48.45&23.7
\\
 InternLM2-chat-7B 
& 57.87& 67.16& 27.43
& 74.76& 82.16& 61.92
& 51.22& 53.92&15.12
\\
 GPT-J-6B 
& 55.76& 53.53& 73.27
& 62.06& 57.6& 86.03
& 50.96& 50.67&63
\\
 Opt-6.7B & 47.3& 47.18& 63.45
& 52.18& 50.87& 73.27
& 49.74& 49.74&67.75
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/new_prompt_gen_total/sub_gen_health.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: Health and Privacy}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclcclllllll}
 & \multicolumn{9}{c}{Health and Privacy} & \multicolumn{3}{c}{Variants}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{Phy}& \multicolumn{3}{c}{Men}&  \multicolumn{3}{c}{Pri} & \multicolumn{3}{c}{}\\
        ~ & acc& P&R& acc& P& R& acc& P&R & acc& P&R \\ 
        \midrule
		\multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 53.67& 53.77&41.68
& 56.52& 57.26& 47.55
& 72.21& 68.67&79.42
& 82.28& 74.89&98.44
\\
		Llama3-ChatQA-1.5-70B & 49.71& 48.55&38.27
& 50.26& 49.62& 39.39
& 57.27& 56.71&53.52
& 65.71& 65.39&70.34
\\
		Qwen1.5-72B-Chat & 52.52& 53.23&29.27
& 61.69& 65.36& 47.93
& 66.77& 69.11&58.02
& 77.32& 77.08&79.36
\\
		Opt-66B & 55.04& 52.83&80.77
& 55.04& 52.98& 80.6
& 54.18& 52.08&79.37
& 52.96& 52.93&74.82
\\
		\multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 45.32& 31.65&9.67
& 42.07& 13.81& 3.36
& 63.46& 68.8&46.32
& 83.11& 81.82&86.2
\\
 Opt-30B & 51.07& 50.19& 72.48
& 52.39& 51.25& 74.99
& 52.79& 51.15&76.28
& 50.32& 51.12&69.41
\\
 \multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 60.87& 63.72& 47.41
& 60.28& 63.46& 46.34
& 66.77& 68.53&59.35
& 80.66& 77.82&87.08
\\
 Qwen1.5-14B 
& 40.77& 33.12& 19.91
& 49.01& 47.9& 36.66
& 57.74& 57.16&54.29
& 78.3& 71.88&94.71
\\
 Baichuan2-13B-Chat 
& 51.31& 50.69& 41.06
& 54.58& 54.69& 47.74
& 63.47& 61.95&65.74
& 71& 68.55&80.22
\\
 Ziya2-13B-Chat 
& 54.63& 53.06& 67.68
& 49.84& 49.34& 57.84
& 49.48& 48.61&57.35
& 65.04& 61.16&86.99
\\
		Opt-13B & 51.13& 50.24&71.14
& 52.38& 51.25& 73.5
& 51.05& 49.93&71.18
& 50.75& 51.44&68.89
\\
 \multicolumn{13}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 48.84& 47.53& 38.46
& 54.69& 54.53& 50.38
& 64.86& 62.34&71.08
& 78.77& 71.42&97.7
\\
 DeepSeek-LLM-7B-Chat 
& 61.91& 63.19& 54.17
& 59.62& 61.26& 49.55
& 59.33& 60.43&48.79
& 84.06& 77.1&98.01
\\
 GLM-4-9B-Chat 
& 50.47& 47.63& 6.69
& 48.23& 25.91& 2.51
& 64.94& 82.91&35.7
& 80.28& 91.06&68.23
\\
 Mistral-7B 
& 57.97& 57.99& 53.07
& 62.06& 61.7& 61.38
& 69.23& 66.15&76.01
& 78.65& 72.58&93.78
\\
 Qwen1.5-7B-Chat 
& 63.27& 59.3& 80.93
& 67.77& 62& 89.89
& 66.92& 61.17&88.58
& 73.16& 65.87&98.88
\\
 Yi-1.5-9B-Chat 
& 58.16& 57.12& 60.29
& 62.94& 60.92& 69.93
& 69.52& 64.56&83.48
& 71.93& 67.57&86.94
\\
 Llama3-ChatQA-1.5-8B 
& 58.19& 54.79& 86.75
& 61.42& 56.72& 93.01
& 59.14& 55.11&88.98
& 64.98& 59.67&97.7
\\
 Baichuan2-7B 
& 62.35& 65.64& 49.44
& 65.72& 68.7& 56.35
& 54.61& 56.07&33.49
& 62.83& 68.27&51.42
\\
 InternLM2-chat-7B 
& 52.23& 54.99& 16.29
& 54.28& 61.2& 20.7
& 54.78& 61.06&21.03
& 71.67& 82.33&56.97
\\
 GPT-J-6B 
& 59.84& 56.38& 81.39
& 61.36& 57.43& 84.26
& 57.2& 54.47&76.27
& 57.71& 56.54&75.55
\\
 Opt-6.7B & 51.2& 50.29& 71.14
& 52& 51.02& 72.62
& 50.69& 49.69&70.34
& 49.19& 50.31&65.71
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/new_prompt_gen_total/sub_gen_illegal.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The performance on sub category: illegal activities}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lcclccllll}
 & \multicolumn{9}{c}{Illegal activities}\\
		\toprule
		\multirow{2}*{Model} & \multicolumn{3}{c}{PI}& \multicolumn{3}{c}{POR}&  \multicolumn{3}{c}{CRI}\\
        ~ & acc& P&R& acc& P& R& acc& P&R\\ 
        \midrule
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size > 65B }}}\\
		DeepSeek-LLM-67B-Chat & 82.76& 77.07&97.32
& 81.55& 74.69& 96.94
& 78.95& 71.76&93.38
\\
		Llama3-ChatQA-1.5-70B & 69.93& 70.35&77.52
& 70.67& 68.36& 80.07
& 73.89& 67.9&87.73
\\
		Qwen1.5-72B-Chat & 73.3& 77.62&71.74
& 80.95& 78.65& 86.41
& 82.67& 77.53&90.56
\\
		Opt-66B & 58.26& 58.38&81.86
& 55.98& 54.93& 80.69
& 54.79& 52.27&81.1
\\
		\multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{Size $\approx$ 30B }}}\\
		Yi-1.5-34B-Chat & 77.28& 81.7&75.11
& 83.83& 82.11& 87.61
& 80.08& 79.02&80.33
\\
 Opt-30B & 54.75& 56.36& 75.18
& 52.88& 52.97& 74.33
& 51.57& 50.1&74.16
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{10B < Size < 20B }}}\\
 InternLM2-Chat-20B 
& 84.87& 81.2& 94
& 83.44& 78.92& 92.46
& 78.16& 74.96&82.68
\\
 Qwen1.5-14B 
& 79.37& 74.44& 94.65
& 78.11& 71.87& 94.23
& 75.02& 68.52&89.79
\\
 Baichuan2-13B-Chat 
& 74.58& 72.64& 85.65
& 74.21& 70.25& 86.41
& 69.22& 65.44&77.55
\\
 Ziya2-13B-Chat 
& 61.77& 61.78& 78.31
& 62.22& 59.71& 81.42
& 60.83& 56.81&80.87
\\
		Opt-13B & 53.39& 55.65&71.5
& 53.76& 53.58& 74.62
& 50.87& 49.61&71.2
\\
 \multicolumn{10}{l}{\cellcolor[HTML]{EFEFEF}\textit{\textbf{5B < Size < 10B }}}\\
		\bottomrule
 Gemma-1.1-7B 
& 75.97& 72.46& 90.23
& 78.51& 71.39& 97.15
& 74.71& 67.76&91.49
\\
 DeepSeek-LLM-7B-Chat 
& 83.2& 78.77& 94.71
& 81.63& 76.28& 93.21
& 72.09& 69.8&74.92
\\
 GLM-4-9B-Chat 
& 87.92& 93.45& 83.73
& 90.34& 92.97& 87.89
& 90.43& 92.19&87.75
\\
 Mistral-7B 
& 75.74& 73.59& 86.58
& 78.51& 72.61& 93.4
& 78.26& 70.6&94.66
\\
 Qwen1.5-7B-Chat 
& 73.54& 68.21& 96.39
& 73.25& 65.99& 98.91
& 72.07& 63.57&99.51
\\
 Yi-1.5-9B-Chat 
& 74.82& 71.19& 90.4
& 75.01& 69.11& 92.87
& 75.97& 67.61&96.93
\\
 Llama3-ChatQA-1.5-8B 
& 65.43& 62.01& 94.49
& 63.68& 59.12& 94.97
& 62.52& 56.72&96.29
\\

 Baichuan2-7B 
& 58.22& 67.81& 44.34
& 59.06& 65.02& 44.23
& 66.75& 68.59&58.19
\\
 InternLM2-chat-7B 
& 64.84& 81.19& 46.23
& 73.01& 83.09& 59.65
& 67.09& 77.14&45.88
\\
 GPT-J-6B 
& 60.28& 60.52& 78.07
& 59.68& 57.85& 79.32
& 59.78& 55.86&81.81
\\
 Opt-6.7B & 52.87& 55.31& 70.43
& 51.41& 52.02& 70.03
& 51.04& 49.72&71.41
\\
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	% \hspace{2.5mm}
	% \begin{minipage}{0.49\linewidth}	
	% 	\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
	% 	\makeatletter\def\@captype{table}
	% 	\small
	% 	\centering
	% 	\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
	% 	\toprule
	% 	\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
	% 	~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
	% 	\midrule
	% 	Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
	% 	Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
	% 	InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
	% 	Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
	% 	Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
	% 	ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
	% 	Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
	% 	Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
	% 	\bottomrule
	% 	\end{tabular}}
	% 	\label{tab3}
	% \end{minipage}
	% \vspace{-1.0em}
\end{table}

==> table/sub.tex <==
\begin{table}[t]
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The 0/3-shot average accuracy (\%) on the validation split and test split.}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.1mm}{\begin{tabular}{lccccll}
		\toprule
		\multirow{2}*{Model} & \multicolumn{2}{c}{Val} & \multicolumn{2}{c}{Test} & & \\
        ~ & 0-shot & 3-shot & 0-shot & 3-shot   & &\\ 
        \midrule
		GPT4  & 55.66 & 54.63 & 55.80 & 54.69  & &\\
		Qwen1.5-72B  & 56.33 & 58.17 & 56.47 & 58.10  & &\\
		Yi1.5-34B & 57.71 & 59.72 & 57.34 & 60.16  & &\\
		Qwen1.5-32B & 54.94 & 57.85 & 55.15 & 57.64  & &\\
		InternLM2-20B & 47.17 & 48.37 & 47.17 & 47.32  & &\\
		Baichuan2-13B & 32.66 & 42.16 & 31.53 & 41.50  & &\\
		Llama3-8B  & 26.72 & 37.91 & 26.61 & 38.01  & &\\
		ChatGLM3-6B-Base & 47.34 & 47.90 & 46.07 & 47.28  & &\\
		\bottomrule
		\end{tabular}}
		\label{tab2}
	\end{minipage}
	\hspace{2.5mm}
	\begin{minipage}{0.49\linewidth}	
		\captionof{table}{The 0/3-shot average accuracy (\%) of base model and chat model on the test split.}
		\makeatletter\def\@captype{table}
		\small
		\centering
		\setlength{\tabcolsep}{1.4mm}{\begin{tabular}{lcccc}
		\toprule
		\multirow{2}*{Model} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Chat} \\
		~ & 0-shot & 3-shot & 0-shot & 3-shot  \\ 
		\midrule
		Yi1.5-34B & 57.34 & 60.16 & 58.99 & 57.48 \\
		Qwen1.5-32B & 55.15 & 57.64 & 59.87 & 58.80 \\
		InternLM2-20B & 47.17 & 47.32 & 48.19 & 45.49 \\
		Baichuan2-13B & 31.53 & 41.50 & 40.74 & 44.60 \\
		Llama3-8B  & 26.61 & 38.01 & 42.04 & 41.73 \\
		ChatGLM3-6B & 46.07 & 47.28 & 30.79 & 27.27 \\
		Gemma-2B  & 24.54 & 28.17 & 34.38 & 33.72 \\
		Qwen1.5-1.8B & 35.60 & 37.69 & 37.50 & 35.78 \\
		\bottomrule
		\end{tabular}}
		\label{tab3}
	\end{minipage}
	\vspace{-1.0em}
\end{table}
